A Visualization System for Hexahedral Mesh Quality Study

In this paper, we introduce a new 3D hex mesh visual analysis system that emphasizes poor-quality areas with an aggregated glyph, highlights overlapping elements, and provides detailed boundary error inspection in three forms. By supporting multi-level analysis through multiple views, our system effectively evaluates various mesh models and compares the performance of mesh generation and optimization algorithms for hexahedral meshes.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> contents/5-Applications-removed.tex <==
\section{Applications}
In this section, we apply our system to support two common tasks in the mesh generation and optimization, i.e., (1) the inspection of the quality improvement using a specific optimization algorithm and (2) the comparison of the performance of different mesh generation algorithms.

\paragraph{Comparison of different 3D hex mesh generation techniques. }
In this section, we conduct three sets of comparison of different hex-mesh generation techniques with our system using three different models, respectively. The first experiment is shown in Figure \ref{fig:app3D_1}. By using aggregated glyphs and feature edge filtering, we can see that two techniques have significantly different results on the circular boundary. In Figure \ref{fig:app3D_1} (a), no highlighted glyphs are at the right top plane, but three glyphs are at the front of the circular shape. However, in Figure \ref{fig:app3D_1} (b), a large number of glyphs appear at the top of the circular shape. And there is a small cluster on the back end. Then, by comparing the feature edges of those two mesh, we can see that the structure of this model under the current threshold is almost the same. The structure can indicate that those two techniques may have a similar strategy of boundary generation. In conclusion, by comparison those two meshes by using the proposed system, we can say that the two techniques have similar performance of generating high quality boundary cells, and the technique used to generate the mesh shown in Figure \ref{fig:app3D_1} (b) is not good for generating high quality cells on the circular plane.
\begin{figure}[th]
\centering
\subfloat[rkm012-1-Fu2016]{\includegraphics[width=0.49\columnwidth]{figures/Cut-enhanced-2020-Fu1206.png}}
\hfill
\subfloat[rkm012-1-proposed]{\includegraphics[width=0.49\columnwidth]{figures/Cut-enhanced-2020-ours.png}}
\caption{Comparison of two hex-meshes generated using two different techniques. For both visualization, we set $r_{max}=1$, $r_{dmin}=0.5$, and $e_{qmax}= 0.85$.}
\label{fig:app3D_1}
\end{figure}

In experiments 2, we compare two polycut techniques by using the bunny model. Through the feature edges visualization, we can see that the numbers of cells of the two models are different, but then, through the aggregate glyphs we see that their structures and clustering positions are relatively similar. For example, there are some clusters between the ears and the two front legs. However, the number of displayed feature edges shows that the quality of Figure \ref{fig:app3D_2} (a) is better than the quality of Figure \ref{fig:app3D_2} (b), because fewer feature edges are shown when the threshold values are identical. In the further, technique (b) may be improved by optimizing the small elements along the structure.

\begin{figure}[th]
\centering
\subfloat[bunny]{\includegraphics[width=0.49\columnwidth]{figures/Polycube-2016.png}}
\hfill
\subfloat[bunny]{\includegraphics[width=0.49\columnwidth]{figures/Polycut-2013.png}}
\caption{The comparison of two different polycut approaches for the bunny model. (a) $r_{max}=1$, $r_{dmin}=0.2$, and $e_{qmax}= 0.9$ (b) $r_{max}=0.01$, $r_{dmin}=0.002$, and $e_{qmax}= 0.9$.}
\label{fig:app3D_2}
\end{figure}

In experiment 3, both meshes show a lot of clusters, but since no glyphs are highlighted, we believe that the element quality of the cluster region is good for both meshes. By comparing the two filtered feature edges, we can see that Figure \ref{fig:app3D_3} (b) has clearer edge structure than (a). This indicates that the quality of the mesh in Figure \ref{fig:app3D_3} (b) is relatively better than the one in (a). Figure \ref{fig:app3D_3} (a) can be improved in areas where the boundaries change drastically.

\begin{figure}[th]
\centering
\subfloat[bumpy torus]{\includegraphics[width=0.48\columnwidth]{figures/PolyCube Deformation-2011.png}}
\hfill
\subfloat[bumpy torus]{\includegraphics[width=0.48\columnwidth]{figures/Complex Shapes-2014.png}}
\caption{The comparison of two bumpy torus hex-meshes. Both visualizations $r_{max}=0.01$, $r_{dmin}=0.04$, and $e_{qmax}= 0.8$.}
\label{fig:app3D_3}
\end{figure}

==> contents/6-UserCaseAndEvaluation-old.tex <==
\section{Evaluation}
\label{sec:evaluation}

We integrate the above comprehensive visualization techniques into one unified system with two separate windows, i.e., the Mesh Quality Analysis Window, and the Boundary Error Analysis Window. We applied our system to analyze the quality of the hex-meshes included in the database of HexaLab \cite{bracci2019hexalab} and from the hex-mesh structure simplification work \cite{gao2017robust}.



\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{figures/new_pipline.png}
\caption{A use case of our system for the analysis of a hex-mesh quality.}
\label{fig:usecase}
\end{figure*}

The process of using our system to analyze a hex-mesh is as follows.
After loading a hex-mesh, the Mesh Quality Analysis window displays the wire-frame of the mesh, the distribution of individual element quality, and an interactive bar chart ranking vertex quality (Figure \ref{fig:usecase} (a)). To locate poor-quality elements, glyph representation is activated, using aggregated glyphs to prevent clutter (Figure \ref{fig:usecase}(b)). By focusing on the regions with poor quality, the user can select a large aggregated glyph corresponding to a small cluster and inspect the area in the sub-region view (Figure \ref{fig:usecase}(c), top). A bad-quality vertex can be chosen for detailed inspection, revealing its Jacobian configurations and connectivity configuration (Figure \ref{fig:usecase}(c), middle and bottom). This multi-level, multi-perspective mesh quality analysis process efficiently identifies and analyzes mesh quality issues.

\begin{figure}[th]
\centering
\subfloat[HexaLab]{\includegraphics[width=0.32\columnwidth]{figures/kitten_hexalab.png}}
\hfill
\subfloat[focus + context volume randering]{\includegraphics[width=0.32\columnwidth]{figures/kitten_hexaVol.png}}
\hfill
\subfloat[our method]{\includegraphics[width=0.32\columnwidth]{figures/kitten_our.png}}
\caption{Comparison of the quality visualization using HexaLab (a), focus+context volume rendering (b), and our methods (c) for a teddy bear hex-mesh (top row) and a kitten hex-mesh (bottom), respectively.}
\label{fig:QualityOverviewCompare}
\end{figure}



\paragraph{Element quality analysis.}
To evaluate the effectiveness of our proposed visual encoding, we compare our visualizations of a few meshes with those shown by HexaLab \cite{bracci2019hexalab} and the focus+context volume rendering \cite{neuhauser2021interactive}, respectively. Since the other two approaches do not explicitly support the boundary error visualization, our comparison focuses on the element quality analysis and the effective revelation of low-quality elements with different sizes. 
Figure \ref{fig:Motivationcompare} compares the quality visualization of a warrior hex-mesh using the three approaches. Both HexaLab and the focus+context volume rendering cannot effectively reveal the bad elements at the tips of those protruded features. In contrast, our aggregated glyphs not only highlight those places but also convey how severe the element quality is in those regions via the sizes of the glyphs. 

Figure \ref{fig:QualityOverviewCompare} compares the quality visualization of a kitten hex-mesh using the three methods, respectively. From this comparison, we see that among the three approaches, the focus+context volume rendering can provide the smoothest visual representation of the mesh quality. However, if the two areas have a similar quality, the volume rendering will not effectively distinguish their difference as humans cannot accurately tell the difference between similar colors if they are not next to each other (e.g., the back and the left ear of the kitten). Also, one may think the quality of the elements in the left ear of the kitten is worse than those in the right ear because they look more prominent.  In contrast, HexaLab can provide a more accurate reading on the element quality by filtering. That is, the remaining elements after filtering all have quality lower than a user-specified threshold. However, the difference among these remaining elements is hard to discern (e.g., it is hard to decide which elements are worse than the other in Figure \ref{fig:QualityOverviewCompare}(a)). Also, depending on the threshold, other less optimal areas may not be captured (e.g., the top of the kitten and the middle of the tail of the kitten). As a comparison, our aggregated glyph visualization retains most of the areas with bad-quality elements and allows a more accurate interpretation of the quality difference among these regions using the sizes of the glyphs. For example, the quality of elements at the back of the neck of the kitten (represented by a big green glyph) is worse than those at the back that are prominent in both HexaLab and volume-rendering visualization. Similarly, there is a ring of bad-quality elements at the top of the head of the kitten that is not emphasized by the other two methods due to their small sizes.


% \begin{wrapfigure}{r}{0.35\columnwidth}
% \hspace{-0.2in}
% % \vspace{-0.in}
%   \label{fig:project}\includegraphics[width=0.4\columnwidth]{figures/3D_intersection.png}
% \end{wrapfigure}

\begin{figure}[t]
\centering
\subfloat[Overlapping vertex]{\includegraphics[width=0.45\columnwidth]{figures/overlaping_3d.png}}
\hfill
\subfloat[Intersecting cell]{\includegraphics[width=0.45\columnwidth]{figures/intersection_3d.png}}
\caption{Overlapping vertices and intersecting cells in a 3D view are difficult to be distinguished, as the lines obstruct their visibility.}
\label{fig:intersection_overlapping_3d}
\end{figure}

\paragraph{Overlapping cells analysis.} %\guoning{To complete}
\autoref{fig:intersection_overlapping_3d} shows an example of overlapping and intersection elements in a fandisk mesh. As can be observed in this figure, the overlapping vertices \autoref{fig:intersection_overlapping_3d}(a) are difficult to notice without the additional glyph design. A similar observation can be made for the intersection elements \autoref{fig:intersection_overlapping_3d}(b). By using the proposed method, the cells involved in the intersection are highlighted, with each element colored distinctly, and an arrow is created to indicate the intersection vertices.

\paragraph{Boundary error analysis.} To analyze the boundary error of a mesh, the system loads the original and target meshes into the Boundary Error Analysis Window, as shown in Figure \ref{fig:usecase} bottom row, to provide comprehensive visualization. In the window, the main view displays overlapping surfaces, but occlusion hides some error distributions. The UV map provides a comprehensive overview without requiring the user to select different viewpoints, though it lacks 3D context like sharp features and corners.
The boundary error distribution doesn't show a consistent pattern near specific feature types. For instance, concave areas corresponding to limb-torso conjunctions can exhibit both positive and negative errors. Larger errors typically occur where the surface has a significant curvature, as these areas are challenging to preserve. the sorted error value bar chart enables quick identification of vertices with large boundary errors and their nature.

Additional results can be found in the supplemental document.




==> contents/7-Conclusion-old.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we present a new visual analysis system for the study of the quality of 3D hexahedral meshes. Our system offers a number of simple but effective visual encoding techniques to reveal small elements with low quality and highlight overlapping elements that are difficult to capture with the existing visualization approaches. In addition, we provide a comprehensive visualization of the boundary errors that are often ignored by the existing tools. Our system also provides a multi-view capability to support a multi-level inspection of the mesh quality. The evaluation shows that our system out-performs the existing tools in the tasks of locating small elements with low quality, finding overlapping elements in the mesh, and studying boundary error configurations. Our tool has also been applied for the comparison of a number of mesh generation and mesh optimization techniques to demonstrate its use in practice. 

Despite offering a more comprehensive visual analysis of the mesh quality than existing tools, there are still a few limitations of our current system.
First, the construction of our aggregated glyphs requires performing collision detection among nearby spheres, which is slow. In general, for hex-meshes with 10K elements or less, the aggregated glyphs can be constructed in 1 minute. For meshes with 10K to 25K elements, our method constructs the aggregated glyphs in 3 minutes.
Second, our system does not suggest the ideal configuration for a comparative study of the bad-quality elements. 
Third, our arrow placement strategy for highlighting overlapping elements may still produce overlapping arrows in small regions with many overlapping elements. 
% Fourth, the base complex visualization can be integrated into our system to provide more guidance for mesh quality exploration. 
Finally, the quality of the simulations run on the given meshes can be visualized to help study the correlation between the mesh quality and simulation quality \cite{gao2017evaluating} directly. It is worth mentioning that some models may not be successfully unfolded due to the limitation of the used UV unfolding algorithm. Future work will focus on addressing these limitations and improving the unfolding process for boundary error analysis.

\clearpage

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> vis-23-lei-sup/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> vis-23-lei-sup/contents/1-Abstract.tex <==
% \lei{boundary error could be analyzed in three different view and level.}
\abstract{
The supplemental shows the extension of the proposed system. the proposed system can be also applied to the Quad mesh analysis.
}




==> vis-23-lei-sup/contents/2-FeatureEdgeFilter.tex <==
\section{feature edge filtering}
\begin{wrapfigure}{r}{0.25\columnwidth}
\hspace{-0.2in}
\vspace{-0.in}
  \label{fig:project}\includegraphics[width=0.27\columnwidth]{figures/featureEdgeFilter.jpg}
\end{wrapfigure}
To visualize the distribution of poor-quality elements, we provide a \emph{feature edge filtering} functionality along with the aggregated glyphs. In particular, we emphasize the edges that connect two vertices whose surrounding elements' quality is lower than a user-specified threshold, while de-emphasizing other edges (see the inset figure to the right for an illustration).

==> vis-23-lei-sup/contents/3-ParametersImpact.tex <==
\section{Impact of the parameters}
\paragraph{Impact of the parameters.} There are a number of important user-controllable parameters that will impact the effect of visual encoding. They are the maximum sphere radius $r_{max}$, the minimum displayed sphere radius $r_{dmin}$, and the maximum quality of feature edges $e_{qmax}$.

\noindent\emph{maximum sphere radius.} After numerous experiments, we identified an empirical percentage of the maximum sphere radius. The percentage is the $50\%$ of average edge length. If the radius is set too large, the glyph will occupy a large space. But if the radius is too small, glyphs may be too small to highlight regions with bad-quality elements.

\noindent\emph{minimum displayed sphere radius.} In most cases, we set $r_{dmin}=10\% \times r_{max}$, which is sufficient to filter out the glyphs that are too small (i.e., corresponding to regions with good quality elements).

\noindent\emph{maximum quality of feature edges.} Based on our experiments, we found that $e_{qmax}=0.2 + q_m$ usually yields good feature edge structure, where $q_m$ is the middle value of all vertex quality values. Figure \ref{fig:app3D_rockerarm} compares two meshes for the same model with different feature edge thresholds.  
\begin{figure}[th]
\centering
\subfloat[rockerarm-m1]{\includegraphics[width=0.33\columnwidth]{figures/rockerarm-restricted-Field-2012.png}}
\hfill
\subfloat[rockerarm-m2]{\includegraphics[width=0.33\columnwidth]{figures/rockerarm-PolyCube-Map-Construction-2016.png}}
\hfill
\subfloat[rockerarm-m2]{\includegraphics[width=0.33\columnwidth]{figures/rockerarm_0.85-PolyCube-Map-Construction-2016.png}}
\caption{Feature edge based quality summary representation for two rockerarm hex-meshes, i.e., the mesh shown in (a) is different from the mesh in (b) and (c). Also, we set $e_{qmax}= 0.8$ for (a) and (b) whose corresponding feature edges reveal the structure difference between the two meshes. $e_{qmax}= 0.85$ for (c) which shows the same mesh of (b) with different sets of filtered feature edges.}
\label{fig:app3D_rockerarm}
\end{figure}

\subsection{Comparison of different 3D hex mesh generation techniques. }

In this section, we conduct three sets of comparisons of different hex-mesh generation techniques with our system using three different models, respectively. The first experiment is shown in Figure \ref{fig:app3D_1}. By using aggregated glyphs and feature edge filtering, we can see that the two techniques have significantly different results on the circular boundary. In Figure \ref{fig:app3D_1} (a), no highlighted glyphs are at the right top plane, but three glyphs are at the front of the circular shape. However, in Figure \ref{fig:app3D_1} (b), a large number of glyphs appear at the top of the circular shape. And there is a small cluster on the back end. Then, by comparing the feature edges of those two meshes, we can see that the structure of this model under the current threshold is almost the same. The structure can indicate that those two techniques may have a similar strategy of boundary generation. In conclusion, our comparison of the two meshes using the proposed system indicates that both techniques exhibit similar performance in generating high-quality boundary cells. However, the method employed to produce the mesh shown in Figure \ref{fig:app3D_1} (b) is less effective in generating high-quality cells on the circular plane.
\begin{figure}[th]
\centering
\subfloat[rkm012-1-Fu2016]{\includegraphics[width=0.49\columnwidth]{figures/Cut-enhanced-2020-Fu1206.png}}
\hfill
\subfloat[rkm012-1-proposed]{\includegraphics[width=0.49\columnwidth]{figures/Cut-enhanced-2020-ours.png}}
\caption{Comparison of two hex-meshes generated using two different techniques. For both visualization, we set $r_{max}=1$, $r_{dmin}=0.5$, and $e_{qmax}= 0.85$.}
\label{fig:app3D_1}
\end{figure}

In experiment 2, we compare two polycut techniques using the bunny model. Through the feature edges visualization, we can see that the numbers of cells of the two models are different, but then, through the aggregate glyphs we see that their structures and clustering positions are relatively similar. For example, there are clusters between the ears and the two front legs. However, the number of displayed feature edges shows that the quality of Figure \ref{fig:app3D_2} (a) is better than the quality of Figure \ref{fig:app3D_2} (b), because fewer feature edges are shown when the threshold values are identical. In the future, technique (b) may be improved by optimizing the small elements along the structure.

\begin{figure}[th]
\centering
\subfloat[bunny]{\includegraphics[width=0.49\columnwidth]{figures/Polycube-2016.png}}
\hfill
\subfloat[bunny]{\includegraphics[width=0.49\columnwidth]{figures/Polycut-2013.png}}
\caption{The comparison of two different polycut approaches for the bunny model. (a) $r_{max}=1$, $r_{dmin}=0.2$, and $e_{qmax}= 0.9$ (b) $r_{max}=0.01$, $r_{dmin}=0.002$, and $e_{qmax}= 0.9$.}
\label{fig:app3D_2}
\end{figure}

In experiment 3, both meshes show a lot of clusters, but since no glyphs are highlighted, we believe that the element quality of the cluster region is good for both meshes. By comparing the two filtered feature edges, we can see that Figure \ref{fig:app3D_3} (b) has a clearer edge structure than (a). This indicates that the quality of the mesh in Figure \ref{fig:app3D_3} (b) is relatively better than the one in (a). Figure \ref{fig:app3D_3} (a) can be improved in areas where the boundaries change drastically.

\begin{figure}[th]
\centering
\subfloat[bumpy torus]{\includegraphics[width=0.48\columnwidth]{figures/PolyCube Deformation-2011.png}}
\hfill
\subfloat[bumpy torus]{\includegraphics[width=0.48\columnwidth]{figures/Complex Shapes-2014.png}}
\caption{The comparison of two bumpy torus hex-meshes. Both visualizations $r_{max}=0.01$, $r_{dmin}=0.04$, and $e_{qmax}= 0.8$.}
\label{fig:app3D_3}
\end{figure}

==> vis-23-lei-sup/contents/4-QuadMesh.tex <==
\section{Quad mesh quality visualization}

It is known that the quality of quadrilateral meshes impacts the accuracy and efficiency of various finite element simulations \cite{gao2017evaluating,zhang20053d}. Therefore, a common goal of all quad mesh generation and optimization algorithms is to produce high-quality meshes \cite{BommesLPPSTZ13}.

\subsection{Comparison of 2D quad meshes before and after optimization}

% \paragraph{Comparison of 2D quad meshes before and after optimization. } 
We use our system to compare the quality of two quad meshes before and after optimization. Figure \ref{fig:app2d_maze3} shows such an example. In this example, a maze wheel quad mesh is used. The original mesh and its quality are shown in  Figure \ref{fig:app2d_maze3} (a), while the optimized mesh using the method by Akram et al. \cite{akram2021embedded} is shown in (b). We can immediately notice the reduction of both the number of aggregated glyphs and the sizes of the individual glyphs in (b) when compared to those in (a). This suggests the improvement of the overall element quality of the entire mesh. To study the boundary error, we turn on the Boundary Error Analysis Window as shown in Figure \ref{fig:2DBoundaryErrorInterface}. Since this mesh consists of three closed boundary curves, including the out-most boundary consisting of most boundary vertices and two small holes. The collated error plot shown in the lower right of the figure suggests that most parts of the boundary are preserved well in the optimized mesh, especially the two holes as their error ranges are smaller than the range of the outer boundary (e.g., the red section). Indeed, the places with the largest boundary error are on the outer boundary and located at the concave sharp feature. 

\begin{figure}[th]
\centering
\subfloat[before optimization]{\includegraphics[width=0.48\columnwidth]{figures/2Dmaze3.png}}
\hfill
\subfloat[after optimization]{\includegraphics[width=0.48\columnwidth]{figures/2dMaze3_opt.png}}
\caption{The aggregated glyph visualizations for a maze wheel quad mesh before (a) and after optimization (b).}
\label{fig:app2d_maze3}
\end{figure} 

\subsection{Boundary error analysis for 2D meshes}
For 2D meshes with boundaries, boundaries need to be extracted before calculating the boundary difference between the original (i.e., the output of some re-meshing or optimization algorithms) and the reference (i.e., the input mesh whose boundary needs to be preserved) mesh models. After boundary extraction, for each point on the extracted boundaries of the original mesh, the boundary error based on the closest point on the extracted boundaries of the reference mesh is calculated as:
\begin{equation}
b_{error} = \frac{dist(\mathbf{p}_{original}, \mathbf{p}_{reference})}{diag_{reference}}
\end{equation}
where $diag_{reference}$ denotes the diagonal of the bounding box of the reference mesh. 

Our method visualizes the extracted boundaries of the original mesh with color coding and a corresponding boundary error plot for each closed boundary. Note that multiple boundary curves may exist for models with holes. Each value on the boundary error plot belongs to $\mathbb{R}$, where positive values indicate that the boundary point is outside the reference mesh while negative values identify boundary points that are inside the reference mesh as shown in Figure \ref{fig:2DBoundaryErrorInterface}.

In addition, a collated percentage graph is visualized for all the boundary vertices in the original mesh as illustrated in Figure \ref{fig:2DBoundaryErrorInterface} (bottom right plot). This enables further insight into boundary error by providing an overall representation of the boundary difference between the original and reference meshes. Thus, boundary areas with a maximum difference between original and reference meshes can be quickly identified.

\begin{figure}[!t]
\centering
\includegraphics[width=1.\columnwidth]{figures/2dMaze3_bnd.png}
\caption{Interface for the 2D boundary error visualization. The main view (left) shows the overlapping boundaries of the two meshes\cite{akram2021embedded}. The right views show the error plots for the individual boundary curves. The vertices on each boundary curve are sorted based on their positions on the curve. The bottom right plot shows the error for all boundary vertices, which supports user interaction such as zoom-in, panning, and selection. In this case, a selected boundary section is highlighted in the left main view.}
\label{fig:2DBoundaryErrorInterface}
\end{figure} 





==> vis-23-lei-sup/contents/5-UserFeedback.tex <==
\section{User Feedback}

% how to mark blue for a whole section
To evaluate our proposed system, we created an online user feedback survey using Typeform, a platform providing various features that support the survey's credibility and feasibility. The reasons for conducting an online survey using Typeform are as follows.

Firstly, an online survey platform offers a highly convenient means of data collection, eliminating the need to consider geographical locations and enabling data collection from individuals across various disciplines.

Secondly, the ranking and picture selection features of Typeform reduce the necessity of pre-setting permutations, combinations, and answers. Consequently, this minimizes the potential influence of the designer on participants. For instance, rather than explicitly suggesting where each method needs attention, users can make selections based on their personal judgments.

Thirdly, the one-question-at-a-time display mitigates the issue of users referencing images from other questions while answering the current one.

Lastly, Typeform provides an engaging and visually appealing interface for the survey.

Capitalizing on these features of Typeform, we designed 13 questions for users to evaluate our system. The survey attracted 185 views and received 38 valid submissions. The questions and corresponding results are discussed in the following three sections.


\subsection{Introduction to Hexahedral Meshing}

Given that both the proposed system and the survey cater to more than just mesh experts, we have included a brief introduction prior to the system-related questions. This ensures that participants acquire some foundational knowledge before delving into the main survey questions.

\paragraph{Hexahedral Meshing Introduction} is the first part of this section, which contains two parts. The first part provides a brief explanation of hexahedral meshing. The second part asks participants to indicate whether they are mesh experts.

From the responses, we found that 11 participants identified themselves as mesh experts, while the remaining 27 indicated they did not possess expertise in the field.

\paragraph{Hex Element Shape Analysis} seeks to educate users that an ideal hexahedral element has a regular hexahedral shape (i.e., a regular cube with six equal quad-faces and 90-degree angles between faces). Deviations from this shape, such as highly distorted or skewed elements, can have adverse effects on mesh quality.

Once users have grasped these basic concepts, they are asked to select the element of the worst quality from three options varying from ideal to 45 degrees and finally to a flat corner.

In the responses collected, 73\% of users were able to correctly identify the worst shape.

\subsection{Comparative Analysis: Evaluating Three Different Tools}

This section focuses on the evaluation of three different methods used to analyze hex mesh quality.

\paragraph{Region Ranking} 

In order to evaluate whether our proposed system can assist users in prioritizing different regions, we applied three methods to the same model. Given that the survey does not allow users to manually mark regions, we pre-identified three regions and labeled them for users to rank.

\begin{figure}[th]
\centering
\includegraphics[width=1.\columnwidth]{figures/person_ref.png}
\caption{A Greek Sculpture model from \cite{fu2016efficient} is analyzed by the proposed HQView system. Region 1 contains the lowest mesh quality, 0.25. The mesh quality in Region 2 is between 0.53 to 0.77, but since the region is very crowded, hence the region is also been noticed. Region 3 contains elements with quality from 0.37 to 1.0 since the quality of most elements in this region is lower than 0.69, hence the region is noticeable.}
\label{fig:3D_Region_Ranking}
\end{figure}

Based on the reference image \autoref{fig:3D_Region_Ranking}, which is created by the proposed method, Region 1 contains the poorest quality elements and the globally lowest mesh quality. And Region 2 and Region 3 contain a considerable number of poor-quality elements.

From the survey results, we observed that more than 50\% of the respondents ranked Region 1 as the highest priority for all three methods. However, in Hexalab, 50\% of users ranked Region 3 as the lowest priority. For volumetric context rendering and HQView, the respondents nearly equally divided Region 3 between the second and third rankings. The results indicate that Region 2 can successfully draw the attention of users, despite the mesh over this area being relatively small.

\paragraph{Region Counting}

\begin{figure}[th]
\centering
\includegraphics[width=1.\columnwidth]{figures/fandisk_ref.png}
\caption{A fandisk model from \cite{guo2020cut} is analyzed by the proposed HQView system. This model contains 6 regions characterized by elements of poor quality. With the detail views, each of these regions contains at least one element with a quality value of less than $0.3$}
\label{fig:3D_Region_Count}
\end{figure}

In order to assess the effectiveness of identifying small-sized elements of poor quality, the survey asked participants to identify all regions containing such elements. A reference image, as displayed in \autoref{fig:3D_Region_Count}, reveals that this model includes 6 distinct regions marked by elements of their quality. Upon the detailed sub-region reviews, it is observed that each of these regions has at least one element that falls below a quality score of $0.3$.

The results indicate that Hexalab struggles to clearly depict all regions, with over 78\% of responses ranging between 2 to 4 identified regions. 

The focus+content volume rendering method, on the other hand, can display these regions, but it might lead to confusion among users. The range of regions identified from the focus+context volume rendering ranges from 3 to 9, and no single number of regions was selected by more than 50\% of users. 

Conversely, the proposed method can depict the regions more accurately. The number of regions identified ranged from 3 to 8. More specifically, 50\% of respondents identified 6 regions, and 23.7\% of respondents identified 7 regions.

\paragraph{Region Highlighting}

The main focus of our proposed method is to highlight regions or elements where the size of the element is small, yet the quality is poor.

To assess the effectiveness of this approach, we included two questions in this section to determine if participants find our method better at identifying such regions or elements.

\begin{figure}[th]
\centering
\includegraphics[width=1.\columnwidth]{figures/bunny_ref.png}
\caption{The bunny model is obtained from \cite{gao2016structured}. In this model, the areas with the poorest mesh quality are found at the tip of each ear, where the size of the mesh elements is also particularly small.}
\label{fig:Bunny_Region_Highlighting}
\end{figure}

The first question revolved around a 3D bunny model. Within this model, certain elements, specifically located at the tip of the ears, were identified as being of low quality. Notably, these elements were  small in size. The results demonstrate over 55.3\% of respondents affirmed that our method was superior in detecting these small, low-quality regions within the bunny ears.

\begin{figure}[th]
\centering
\includegraphics[width=1.\columnwidth]{figures/hand_ref.png}
\caption{The hand model is obtained from \cite{gao2016structured}. Within this model, the majority of the mesh components exhibit superior quality. However, a solitary and exceptionally small element located at the tip of the little finger is inconspicuous. Our proposed system emphasizes this region by accentuating the problematic element with a prominently displayed, large glyph.}
\label{fig:hand_Region_Highlighting}
\end{figure}

The second question pertains to a hand model. Within this model, an inconspicuous element located on the little finger exhibits poor quality, registering a score of 0.27 compared to the lowest mesh quality score of 0.18. The size of the element makes the element challenging to discern when using the other two methodologies. Consequently, our tool was chosen by over 50\% of respondents as the optimal solution for this task.

\paragraph{Method Selection}

The last question in this section prompted participants to choose from multiple tools they think are effective at showing degenerate mesh elements.

Each of the three methods gets comparable responses. However, it's crucial to underline that the first option actually fails to accurately represent where the degenerate mesh elements are hidden by an edge.

The other three options have the ability to locate the regions that contain degenerate mesh elements.

\subsection{Sub-System and Component Evolution}
% In addition to the previous mesh element quality analysis system, the proposed method also provides a multi-view boundary error analysis sub-system and an overlapping element indicator component.

The proposed methodology, which incorporates a multi-view boundary error analysis subsystem and a component dedicated to highlighting overlapping elements, is further evaluated by presenting two questions to the users. These questions aim to gather users' ratings regarding the utility of these components.

\paragraph{Boundary Analysis Sub-system}

Over 54\% of the responses rated the introduced components as 3 or higher (on a scale where 3 is neutral), indicating agreement with the usefulness of these additions.


\paragraph{Marks of Overlapping Elements}

Over 55\% of the responses rated the overlapping indicator components as 3 or higher (where 3 is neutral), suggesting agreement with the stated usefulness of these features.

==> vis-23-lei-sup/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

